Using Natural Sentences for Understanding Biases in Language Models

Evaluation of biases in language models is often limited to synthetically generated datasets. This dependence traces back to the need for a prompt-style dataset to trigger specific behaviors of language models. In this paper, we address this gap by creating a prompt dataset with respect to occupations collected from real-world natural sentences present in Wikipedia. We aim to understand the differences between using template-based prompts and natural sentence prompts when studying gender-occupation biases in language models. We find bias evaluations are very sensitive to the design choices of template prompts, and we propose using natural sentence prompts for systematic evaluations to step away from design choices that could introduce bias in the observations.

==> method.tex <==
\section{Causal Mediation Analysis}
\subsection{Causal Attribution}
\begin{definition}[] 
The average causal effect (ACE) of an input neuron $x_i$ with value $a$ on the output neuron $y$ is defined as:
$$ACE = \mathbb{E}[y|do(x_i=a)]-baseline_{x_i}$$
\end{definition}


\subsection{Intervention on GPT model}
From the causal perspective, the language model can be viewed as a mediator between the input and the output. Using intervention, we can identify the causal attribution for specific model components based on granularity: neuron, layer, and path.  
\paragraph{Neuron} Intervention on the value of a specific neuron can be considered as \textit{atomic} intervention. This is equivalent to setting the value of the neuron to a specific value and removing all incoming edges to that neuron. 

\paragraph{Layer} Layer intervention corresponds to applying neuron intervention simultaneously on all the neurons in a specific layer. Layer intervention provides a high level understanding of the how the intervention effect is distributed and is particularly helpful for a large model.
\paragraph{Path} Path intervention provides graphical representation of counterfactual quantities by estimating how treatments affect the response via pathways that end in a
particular edge. A path in a neural network consists of multiple directed edges span from the first layer to the last output layer. A response from the path intervention will be the output value as if the source of the path were set to a specific value. \cite{Shpitser2016CAUSALIW} proposed using recursive function to estimate the causal effect of a path intervention. 



==> tables/perturbation_distibution.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{lrrrrrr}
    \toprule
    {} & \multicolumn{6}{c}{KL}\\
    {} & template\_ & template\_man & template\_mask & template\_original & template\_person & template\_woman \\
    \midrule
    distilgpt2 &     0.104 &        0.528 &         0.051 &             0.187 &           0.149 &         -0.380 \\
    gpt2       &     0.070 &        0.528 &         0.049 &             0.164 &           0.139 &         -0.369\\
    \midrule
    {} & \multicolumn{6}{c}{EMD}\\
    {} & template\_ & template\_man & template\_mask & template\_original & template\_person & template\_woman\\
    distilgpt2 &     0.092 &        0.358 &         0.046 &             0.141 &           0.120 &          0.371 \\
    gpt2 &     0.063 &        0.358 &         0.045 &             0.126 &           0.112 &          0.357 \\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

==> tables/random_prompt.tex <==
% \begin{table}[ht]
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%     & he & she & they \\ 
%     \midrule
%     distilgpt2  &        0.242 &          0.194 \\
%     gpt2-small  &        0.249 &          0.155 \\
%     gpt2-medium &        0.240 &          0.174 \\
%     gpt2-large &        0.314 &          0.203 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Output uncertainty}
%     \label{tab:output_uncertainty}
% \end{table}
